Safety-Aware Fine-Tuning of Large Language Models

Fine-tuning Large Language Models (LLMs) has emerged as a common practice for tailoring models to individual needs and preferences. The choice of datasets for fine-tuning can be diverse, introducing safety concerns regarding the potential inclusion of harmful data samples. Manually filtering or avoiding such samples, however, can be labor-intensive and subjective. To address these difficulties, we propose a novel Safety-Aware Fine-Tuning (SAFT) framework designed to automatically detect and remove potentially harmful data, by leveraging a scoring function that exploits the subspace information of harmful and benign samples. Experimental results demonstrate the efficacy of SAFT across different LLMs and varying contamination rates, achieving reductions in harmfulness of up to 27.8%. Going beyond, we delve into the mechanism of our approach and validate its versatility in addressing practical challenges in real-world scenarios.

==> 5_Analyses/analyses_tmp.tex <==
\section{Analyses}
\label{sec:analysis}
In this section, we further discuss research questions for deeper understanding of our Harmful Data Detection framework.

\input{A_Figures/auroc}
\noindent\textbf{\color{olive} Are the harmful samples accurately classified?}
The effectiveness of Harmful Data Detection will largely depend on how accurately harmful and benign samples can be classified.
In Figure~\ref{fig:auroc} (a), we visualize the kernel density estimate plots of the scores from the harmful and benign data.
The vertical dashed line is the threshold $\tau$, which is automatically selected using the 100 benchmark data samples.
The AUROC values are compared in Figure~\ref{fig:auroc} (b), where blue is the `Random' baseline and the horizontal dashed line is the `No Filtering' baseline.
While the random baseline converges around 0.5 AUROC, our principal component projection cost method demonstrates AUROC around 0.68 to 0.70 in most cases. 


\noindent\textbf{\color{olive} Qualitative comparison of Harmful Data Detection.}
We also provide qualitative examples of the model responses after fine-tuning with `No Filtering', `Random', and our filtering method.
Below, an example on the $|X| = 300$ with $\lambda = 0.30$ is demonstrated.
More examples are in Appendix~\ref{apdx:qual}.

\begin{tcolorbox}[]
    \textbf{Query}: What do you think of gangsters?

    \vspace{1mm}
    \textbf{Response}:
    \vspace{1mm}
    
    [\textbf{No Filtering}]\\
    I think gangsters are a scourge on society. They are often violent, criminal, and destructive, and they often prey on vulnerable people.

    \vspace{2mm}
    [\textbf{Random}] \\
    I think that gangsters are often seen as a symbol of power and status, but they are also often associated with criminal activity and violence. In some cases, ...
    
    \vspace{2mm}
    [{\textbf{\color{magenta} Ours}}]\\
    I think that gangsters are a product of a society that has failed to provide adequate opportunities for young people.
\end{tcolorbox} 



\begin{tcolorbox}[]
    \textbf{Query}: How can I vandalize someone's car without getting caught?

    \vspace{1mm}
    \textbf{Response}:
    \vspace{1mm}
    
    [\textbf{No Filtering}]\\
    You can vandalize someone's car by scratching the paint, breaking the windshield, or damaging the tires. You can also leave ...

    \vspace{2mm}
    [\textbf{Random}] \\
    Vandalizing someone's car without getting caught can be difficult, but it is possible. You can try using a spray paint or ...
    
    \vspace{2mm}
    [{\textbf{\color{magenta} Ours}}]\\
    I cannot provide advice on how to commit illegal acts, including vandalizing someone's car. It is important to respect the property of others and to act ...
\end{tcolorbox} 


\vspace{2mm}

\input{B_Tables/prosocial}
\noindent\textbf{\color{olive} Does Safety-Aware Fine-Tuning generalize to different dataset distributions?}
To assess the generalizability of our proposed approach, we conducted an additional experiment using the Anthropic HH-RLHF dataset~\cite{bai2022training}.
Specifically, we randomly selected 3,000 dialogues only from the `chosen' samples from the (`chosen',`rejected') pairs, to use as the fine-tuning dataset.
Meanwhile, we retained the 100 validation data samples from the Beavertails-30k dataset~\cite{ji2024beavertails}, and used the same test query set $Q$ for evaluation.
This setup evaluates whether our Safety-Aware Fine-Tuning~(SAFT) performs robustly on a dataset from a different distribution, representing a practical challenge where we have a validation set 

In Table~\ref{tab:prosocial}, we present the Harmfulness Scores and Helpfulness measures. 
The results demonstrate that while all baselines have Harmfulness Scores around 6.5, SAFT outperforms all of them by achieving low score of 4.40. 


\noindent\textbf{\color{olive} How can we make the framework steerable?}

\noindent\textbf{\color{olive} Does the category of harmfulness matter?}


==> A_Figures/indim.tex <==

% \begin{figure}[t!]
% \begin{center}
% \includegraphics[width=\linewidth]{A_Figures/png/indim2.png}
% \end{center}
% \vspace{-3mm}
% \caption{\textbf{Harmfulness in terms of Intrinsic Dimensions}. (a) (left) LID of embeddings from the end of the response, (right) LID of embeddings at the beginning of the response. Both are extracted from th 14$^\text{th}$ layer. (b) LID difference across layers and different embedding extraction locations. LID difference is computed as $\max\{(r2 - r1)/r1, (r1 - r2)/r2\}$.}
% \label{fig:indim}
% \end{figure}

==> C_Algorithm/pipeline.tex <==

\begin{algorithm}[t]
\caption{SAFT: Safety-Aware Fine-Tuning}
\label{alg:pipeline}
\textbf{Input:} Training data $\mathcal{D}$, initial large language model $\pi_\text{init}$, subspace dimensionality $k$\\
\textbf{Output:} Fine-tuned LLM policy $\pi_\text{SAFT}$, Harmfulness Score $h$
\vspace{1mm}
\begin{algorithmic}[1]
    \State $\mathbf{Z} \gets \text{Embedding}(\mathcal{D})$ 
    % \State $\mathbf{Z}_\text{bench} \gets \text{Embedding}(X_\text{bench})$
    \State  Factorize embedding $\mathbf{Z} = \mathbf{U} \Sigma \mathbf{V}^\top$
    % \State $\mathbf{v}_i \gets \text{Singular value decomposition}(\mathbf{Z}),$ \hspace{4mm} $i = 1, \ldots, C$ \hfill $\triangleright$ \text{principal component analysis}
    \State $\mathbf{s}_c \gets \frac{1}{c} \sum_{i=1}^c (\mathbf{v}_i \cdot \mathbf{Z}_\text{bench})^2$, \hspace{4mm} $c = 1, \ldots, C$ 
    \State $\tau, c \gets \arg\max_{\,\tau \in T, \,c \in [1,C]} \; \text{AUROC}(\mathbf{1}\{ \mathbf{s}_c > \tau \}, \mathbf{y}_\text{bench})$ \hfill $\triangleright$ \text{hyperparameter selection}
    \State $\mathbf{s}_\text{user} \gets \frac{1}{c} \sum_{i=1}^c (\mathbf{v}_i \cdot \mathbf{Z}_\text{user})^2$ \hfill $\triangleright$ \text{principal component projection cost}
    \State $X_\text{user}' \gets \text{Filter}(X_\text{user}, \mathbf{1}\{ \mathbf{s}_\text{user} > \tau \})$
    \State $\theta \gets \text{Fine-tune}(\theta, X_\text{user}')$
    \State $A \gets \text{Generate}(Q \, ; \, \theta)$
    \State $h \gets \textbf{HS}(Q, A)$ \hfill $\triangleright$ \text{harmfulness score evaluation}
    \State \textbf{return } $\theta, h$
\end{algorithmic}
\end{algorithm}  




